A Convergence Rate for Extended-Source Internal DLA in the Plane

Internal DLA (IDLA) is an internal aggregation model in which particles perform random walks from the origin, in turn, and stop upon reaching an unoccupied site. Levine and Peres showed that, when particles start instead from fixed multiple-point distributions, the modified IDLA processes have deterministic scaling limits related to a certain obstacle problem. In this paper, we investigate the convergence rate of this "extended source" IDLA in the plane to its scaling limit. We show that, if $\delta$ is the lattice size, fluctuations of the IDLA occupied set are at most of order $\delta^{3/5}$ from its scaling limit, with probability at least $1-e^{-1/\delta^{2/5}}$.

==> 7_pointsources.tex <==
\section{Multiple point-sources}

==> 8_conclusion.tex <==
\section{Concluding Remarks}\label{conclusion}
There are a number of possible improvements to the results proven here. Most importantly, it would be interesting to improve the $m^{-3/5}$ bounds on the fluctuations; we expect that fluctuations are truly of order $m^{-1}\log m$, as in the point-source case. Hypothetically, this result could be proven using our technique---the primary obstacle is that we need a stronger version of Lemma \ref{harmoniclemma2}(c), which quantifies how closely $\tilde{H}_\zeta$ approximates a continuum harmonic function. If we were able to get a better $L^1$ convergence rate on $\tilde{H}_\zeta$, the final result would improve accordingly.

Furthermore, it would be interesting to lift some of the hypotheses we set on the flow. However, we imagine that it is less likely our technique would apply without the requirements of a concentrated mass distribution or a smooth flow. Indeed, both hypotheses are necessary to guarantee that $R_0$ is bounded away from 0, and thus that $H_\zeta$ is small enough on the boundary. However, if an independent bound on $\tilde{H}_\zeta$ could be obtained, showing that it satisfies $\tilde{H}_\zeta(z)\leq\frac{1}{md(z,\zeta)-C_2}$ without comparing it to $H_\zeta$, it could be used in place of $H_\zeta$ for both parts of the proof.

There are also closely related settings that have not been studied extensively. An interesting example would be to replace the ``solid'' initial sets $Q^s_i$ with submanifolds of $D_0$. Since these would be zero volume, they could eject particles evenly from all points rather than having a moving source $\bigsqcup_{i}\partial Q^{s_i}_i$. Another example would be a collection of point sources; in fact, the theorem corresponding to Lemma \ref{levinepereslemma} in this setting has already been proved by Levine and Peres \cite[Theorem 1.4]{Levine_2010}, so it would likely not be too difficult to adapt our argument to this case.

Finally, a question we will investigate in the sequel is that of the scaling limits of the fluctuations themselves. Jerison, Sheffield, and Levine \cite{jerison2014} studied this question for same-time fluctuations in the point-source case, and they found that, when the fluctuations are scaled up by a factor of $m^{d/2}$ (in dimension $d$), they have a weak limit in law of a certain Gaussian random distribution. They found a similar result in the case of a discrete cylinder $\mathbb{Z}\times\mathbb{Z}/m\mathbb{Z}$ with source points along a fixed-height circumference \cite{jerison2013internal}; here, they further studied the correlations between fluctuations at different times in the flow. The same question has been studied by Eli Sadovnik \cite{eli16} in the extended-source case, focusing on same-time fluctuations and using harmonic polynomials as test functions; we are interested in strengthening his result to allow smooth test functions and to investigate correlations between fluctuations at different times.

